Partially symmetric monomial codes

A framework of monomial codes is considered, which includes linear codes generated by the evaluation of certain monomials. Polar and Reed-Muller codes are the two best-known representatives of such codes and can be considered as two extreme cases. Reed-Muller codes have a large automorphism group but their low-complexity maximum likelihood decoding still remains an open problem. On the other hand, polar codes have much less symmetries but admit the efficient near-ML decoding. We study the dependency between the code symmetries and the decoding efficiency. We introduce a new family of codes, partially symmetric monomial codes. These codes have a smaller group of symmetries than the Reed-Muller codes and are in this sense "between" RM and polar codes. A lower bound on their parameters is introduced along with the explicit construction which achieves it. Structural properties of these codes are demonstrated and it is shown that they often have a recursive structure.

==> fact0raw.tex <==
	\tikzstyle{tnode}  = [radius=0.05, red, thick, fill=red];
		\tikzstyle{lineP}  = [-, thick,  black];
		\coordinate  (0) at (    0,    0);
		\coordinate  (1) at (	0,		-0.75);
		\coordinate  (2) at (	0,		-1.5);
		\coordinate  (3) at (	0,		-2.25);
		\coordinate  (4) at (	0,		-3);
		\coordinate  (5) at (	0,		-3.75);
		\coordinate  (6) at (	0,		-4.5);
		\coordinate  (7) at (	0,		-5.25);
		
		\coordinate  (8) at (    1.5,     0);
		\coordinate  (9) at (	1.5,	 -0.75);
		\coordinate  (10) at (	1.5,	 -1.5);
		\coordinate  (11) at (	1.5,	 -2.25);
		\coordinate  (12) at (	1.5,	 -3);
		\coordinate  (13) at (	1.5,	 -3.75);
		\coordinate  (14) at (	1.5,	 -4.5);
		\coordinate  (15) at (	1.5,	 -5.25);
		
		\coordinate  (16) at (    3.,    0);
		\coordinate  (17) at (	3.,		-0.75);
		\coordinate  (18) at (	3.,		-1.5);
		\coordinate  (19) at (	3.,		-2.25);
		\coordinate  (20) at (	3.,		-3);
		\coordinate  (21) at (	3.,		-3.75);
		\coordinate  (22) at (	3.,		-4.5);
		\coordinate  (23) at (	3.,		-5.25);	
		
		\coordinate  (24) at (    4.5,    0);
		\coordinate  (25) at (	4.5,	 -0.75);
		\coordinate  (26) at (	4.5,	 -1.5);
		\coordinate  (27) at (	4.5,	 -2.25);
		\coordinate  (28) at (	4.5,	 -3);
		\coordinate  (29) at (	4.5,	 -3.75);
		\coordinate  (30) at (	4.5,	 -4.5);
		\coordinate  (31) at (	4.5,	 -5.25);
		
		\draw  (0)  [tnode] circle;
		\draw  (1) [tnode] circle;
		\draw  (2) [tnode] circle;
		\draw  (3) [tnode] circle;
		\draw  (4) [tnode] circle;
		\draw  (5) [tnode] circle;
		\draw  (6) [tnode] circle;
		\draw  (7) [tnode] circle;
		\draw  (8) [tnode] circle;
		\draw  (9) [tnode] circle;
		\draw (10) [tnode] circle;
		\draw (11) [tnode] circle;
		\draw (12) [tnode] circle;
		\draw (13) [tnode] circle;
		\draw (14) [tnode] circle;
		\draw (15) [tnode] circle;
		\draw (16) [tnode] circle;
		\draw (17) [tnode] circle;
		\draw (18) [tnode] circle;
		\draw (19) [tnode] circle;
		\draw (20) [tnode] circle;
		\draw (21) [tnode] circle;
		\draw (22) [tnode] circle;
		\draw (23) [tnode] circle;
		\draw (24) [tnode] circle;
		\draw (25) [tnode] circle;
		\draw (26) [tnode] circle;
		\draw (27) [tnode] circle;
		\draw (28) [tnode] circle;
		\draw (29) [tnode] circle;
		\draw (30) [tnode] circle;
		\draw (31) [tnode] circle;		
		
		\draw [lineP] (0) -- (24);
		\draw [lineP] (1) -- (25);
		\draw [lineP] (2) -- (26);
		\draw [lineP] (3) -- (27);
		\draw [lineP] (4) -- (28);
		\draw [lineP] (5) -- (29);
		\draw [lineP] (6) -- (30);
		\draw [lineP] (7) -- (31);
		
		
		\draw [lineP] (1) -- (8);
		\draw [lineP] (3) -- (10);
		\draw [lineP] (5) -- (12);
		\draw [lineP] (7) -- (14);
		
		\draw [lineP] (10) -- (16);
		\draw [lineP] (11) -- (17);
		\draw [lineP] (14) -- (20);
		\draw [lineP] (15) -- (21);
		
		\draw [lineP] (20) -- (24);
		\draw [lineP] (21) -- (25);
		\draw [lineP] (22) -- (26);
		\draw [lineP] (23) -- (27);
